VisMin: Visual Minimal-Change Understanding

Fine-grained understanding of objects, attributes, and relationships between objects is crucial for visual-language models (VLMs). Existing benchmarks primarily focus on evaluating VLMs' capability to distinguish between two very similar captions given an image. In this paper, we introduce a new, challenging benchmark termed Visual Minimal-Change Understanding (VisMin), which requires models to predict the correct image-caption match given two images and two captions. The image pair and caption pair contain minimal changes, i.e., only one aspect changes at a time from among the following: object, attribute, count, and spatial relation. These changes test the models' understanding of objects, attributes (such as color, material, shape), counts, and spatial relationships between objects. We built an automatic framework using large language models and diffusion models, followed by a rigorous 4-step verification process by human annotators. Empirical experiments reveal that current VLMs exhibit notable deficiencies in understanding spatial relationships and counting abilities. We also generate a large-scale training dataset to finetune CLIP and Idefics2, showing significant improvements in fine-grained understanding across benchmarks and in CLIP's general image-text alignment. We release all resources, including the benchmark, training data, and finetuned model checkpoints, at https://vismin.net/.

==> neurips/4-VisMin_analysis.tex <==
\section{\bench}

\paragraph{Statistics and Analysis} We develop the \bench using the data generation pipeline, automatic filtering procedures, and human verification, as detailed in Section \ref{sec:dataset_creation}. The benchmark aims to evaluate the fine-grained minimal visual understanding of VLMs in tasks involving minimal changes related to objects, attributes, counting, and spatial relations. Our benchmark dataset comprises a total of 3553 samples, with the training set containing 65605 samples for robust evaluation and effective model training. The benchmark set is distributed across the following categories: 578 samples for object comprehension, 296 samples for attribute recognition, 589 samples for counting, and 621 samples for spatial relations. Fig. \ref{fig:data_analysis} illustrates the distribution of the \bench across primary categories and sub-categories. Please refer to Appendix \textcolor{red}{appendix} for the breakdown of sample numbers across categories and subcategories within the training set.


\paragraph{Compare with other benchmarks}

In Table \ref{tab:benchmark_comparison}, we conduct a comprehensive comparison of VisMin with other similar benchmarks. 1) \textbf{Size}: VisMin's dataset comprises 2084 samples, which is smaller than EqBen's 250K but larger than Winoground's 400. This moderate size ensures a focused and high-quality dataset with significant human verification, balancing comprehensiveness and practicality. 2) \textbf{Visual Minimal Hard Negatives (HN)}: VisMin includes visual minimal hard negatives, which are crucial for evaluating fine-grained visual understanding. This feature is shared with EqBen and SPEC. 3) \textbf{Visual Complexity}: VisMin stands out in visual complexity by editing COCO images, which contain common objects in their natural context. This ensures detailed and realistic images. For counting and spatial relations tasks, we generate an initial image and then edit it, avoiding rule-based captioning and procedural generation methods. This results in highly natural and intricate scenes. SPEC achieves good photo-realism with diffusion-based generation but can deviate from natural scenes due to procedural object placement and background filling. 4) \textbf{Caption Complexity}: VisMin excels with its blend of human-written and LLM-generated captions, unlike benchmarks like What'sUp and SPEC that rely heavily on template-based captions. This diversity enhances linguistic richness and ensures that the captions are more natural and varied. The inclusion of human-written captions from the COCO dataset and LLM-generated texts allows for a comprehensive evaluation of a model's language processing capabilities, making VisMin superior in linguistic diversity. 5) \textbf{Synthetic Human-Approved Content and Photo-Realism}: VisMin uniquely provides human-approved synthetic captions and natural images, ensuring that the synthetic elements are sensible and natural. In summary, VisMin’s commitment to visual complexity, human-approved content sets it apart from other benchmarks.


\input{tables/dataset_analysis}

    \begin{figure}[htbp]
        \centering
        \begin{subfigure}[b]{0.50\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/dataset_analysis/category_distribution.png}
            \caption{Categories and subcategories distribution in benchmark dataset. Training set distribution in \textcolor{red}{Appendix A}.}
            \label{fig:figure1}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.45\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/dataset_analysis/our_benchmark_wordcloud_all.png}
            \caption{Word cloud of our benchmark across different categories}
            \label{fig:figure2}
        \end{subfigure}
        \caption{Our benchmark analysis}
        \label{fig:data_analysis}
    \end{figure}

\section{\bench}

\paragraph{Statistics and Analysis} We develop the \bench using the data generation pipeline, automatic filtering procedures, and human verification, as detailed in Section \ref{sec:dataset_creation}. The benchmark aims to evaluate the fine-grained minimal visual understanding of VLMs in tasks involving minimal changes related to objects, attributes, counting, and spatial relations. Our benchmark dataset comprises a total of 3553 samples, with the training set containing 65605 samples for robust evaluation and effective model training. The benchmark set is distributed across the following categories: 578 samples for object comprehension, 296 samples for attribute recognition, 589 samples for counting, and 621 samples for spatial relations. Fig. \ref{fig:data_analysis} illustrates the distribution of the \bench across primary categories and sub-categories. Please refer to Appendix \textcolor{red}{appendix} for the breakdown of sample numbers across categories and subcategories within the training set.


\paragraph{Compare with other benchmarks}

In Table \ref{tab:benchmark_comparison}, we conduct a comprehensive comparison of VisMin with other similar benchmarks. 1) \textbf{Size}: VisMin's dataset comprises 2084 samples, which is smaller than EqBen's 250K but larger than Winoground's 400. This moderate size ensures a focused and high-quality dataset with significant human verification, balancing comprehensiveness and practicality. 2) \textbf{Visual Minimal Hard Negatives (HN)}: VisMin includes visual minimal hard negatives, which are crucial for evaluating fine-grained visual understanding. This feature is shared with EqBen and SPEC. 3) \textbf{Visual Complexity}: VisMin stands out in visual complexity by editing COCO images, which contain common objects in their natural context. This ensures detailed and realistic images. For counting and spatial relations tasks, we generate an initial image and then edit it, avoiding rule-based captioning and procedural generation methods. This results in highly natural and intricate scenes. SPEC achieves good photo-realism with diffusion-based generation but can deviate from natural scenes due to procedural object placement and background filling. 4) \textbf{Caption Complexity}: VisMin excels with its blend of human-written and LLM-generated captions, unlike benchmarks like What'sUp and SPEC which rely heavily on template-based captions. This diversity enhances linguistic richness and ensures that the captions are more natural and varied. The inclusion of human-written captions from the COCO dataset and LLM-generated texts allows for a comprehensive evaluation of a model's language processing capabilities, making VisMin superior in linguistic diversity. 5) \textbf{Synthetic Human-Approved Content and Photo-Realism}: VisMin uniquely provides human-approved synthetic captions and natural images, ensuring that the synthetic elements are sensible and natural. In summary, VisMin’s commitment to visual complexity, human-approved content sets it apart from other benchmarks.


\input{tables/dataset_analysis}

    \begin{figure}[htbp]
        \centering
        \begin{subfigure}[b]{0.50\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/dataset_analysis/category_distribution.png}
            \caption{Categories and subcategories distribution in benchmark dataset. Training set distribution in \textcolor{red}{Appendix A}.}
            \label{fig:figure1}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.45\textwidth}
            \centering
            \includegraphics[width=\textwidth]{images/dataset_analysis/our_benchmark_wordcloud_all.png}
            \caption{Word cloud of our benchmark across different categories}
            \label{fig:figure2}
        \end{subfigure}
        \caption{Our benchmark analysis}
        \label{fig:data_analysis}
    \end{figure}

==> tables/dataset_size.tex <==

% \begin{table}
%     \begin{minipage}{0.3\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{images/dataset_analysis/category_distribution_wotitle.pdf}
%         \caption{VisMin categories and subcategories.}
%         \label{fig:vismin_subcategories}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{0.68\linewidth}
%     \centering
%         \captionsetup{font=small}
%         \caption{Comparison of benchmarks offering visual hard negatives (HN) across: \faRuler\ size, \faEye\ minimal HN, \faImage\ visual complexity, \faPen\ textual complexity, and \faUserCheck human-approved images and captions. \halfcheckmark: criteria holds for a subset.}
        
%         % \label{tab:benchmark_comparison}
%         \begin{adjustbox}{width=\textwidth}
%         \begin{tabular}{lllp{6cm}lll}
%             \toprule
%             {Benchmark} & {\faRuler} & {\faEye} & {\faImage} & {\faPen} & {\faUserCheck}\faExclamation & {\faUserCheck\faPalette} \\
%             \midrule
%             ImageCoDe~\cite{imagecode} & 2,306 & \halfcheckmark & \textit{Limited video domains, Open Images} & \textit{Free-form (Human)} & \checkmark & \checkmark \\
%             What'sUp (A/B)~\cite{whatsup} & 1,232 & \checkmark & \textit{Household, Tabletop (Spatial Relations)} & \textit{Template} & \checkmark & \checkmark \\
%             Winoground~\cite{winogorund} & 400 & \texttimes & \textit{Expert curated using Getty Images API} & \textit{Free-form (Human)} & \checkmark & \checkmark \\
%             EQBEN~\cite{EqBen} & 250,612 & \checkmark & \textit{Limited video domains, Graphic engine, Synthetic-diffusion}  & \textit{Free-form (Human), Template} & \texttimes & \texttimes \\
%             SPEC~\cite{spec} & 3,000 & \checkmark & \textit{Synthetic-diffusion (limited objects)} & \textit{Template} & \texttimes  & \texttimes \\
%             MMVP~\cite{tong2024eyes} & 150 & \texttimes & \textit{ImageNet, LAIONAesthetics} & \textit{Free-form (Human)} & \checkmark & \checkmark \\
%             \bench (Ours) & 2,084 & \checkmark & \textit{COCO, Synthetic-diffusion} & \textit{Free-form (Human, LLM)} & \checkmark & \checkmark \\
%             \bottomrule
%         \end{tabular}
%         \end{adjustbox}
%         \label{fig:comparison_benchmark}
%     \end{minipage}
%      \vspace{-20pt}
% \end{table}

